Challenging Machine Learning Algorithms in Predicting Vulnerable JavaScript Functions

The rapid rise of cyber-crime activities and the growing number of devices threatened by them place software security issues in the spotlight. As around 90% of all attacks exploit known types of security issues, finding vulnerable components and applying existing mitigation techniques is a viable practical approach for fighting against cyber-crime. In this paper, we investigate how the state-of-the-art machine learning techniques, including a popular deep learning algorithm, perform in predicting functions with possible security vulnerabilities in JavaScript programs. We applied 8 machine learning algorithms to build prediction models using a new dataset constructed for this research from the vulnerability information in public databases of the Node Security Project and the Snyk platform, and code fixing patches from GitHub. We used static source code metrics as predictors and an extensive grid-search algorithm to find the best performing models. We also examined the effect of various re-sampling strategies to handle the imbalanced nature of the dataset. The best performing algorithm was KNN, which created a model for the prediction of vulnerable functions with an F-measure of 0.76 (0.91 precision and 0.66 recall). Moreover, deep learning, tree and forest based classifiers, and SVM were competitive with F-measures over 0.70. Although the F-measures did not vary significantly with the re-sampling strategies, the distribution of precision and recall did change. No re-sampling seemed to produce models preferring high precision, while re-sampling strategies balanced the IR measures.

==> data/alg_params.tex <==
% Table generated by Excel2LaTeX from sheet 'Munka2'
\begin{table*}[htbp]
  \centering
  \caption{The applied parameters for the different machine learning algorithms}
    \begin{tabular}{l|l}
    \textbf{Alg.} & \textbf{Parameters} \\
    \midrule
    \midrule
    DNN$_s$  & layers[2-5], neurons[100,150,200], batch[100], epochs[2,5,10,20], learn rate[0.025,0.05,0.1,0.2,0.3,0.4,0.5] \\
    DNN$_c$  & layers[4-6], neurons[150,200,250], batch[50,100,150], beta[0.0005,0.001,0.002,0.005,0.02], learn rate[0.025,0.05,0.1,0.2,0.3,0.4,0.5] \\
    KNN   & n\_neighbors[6,8,…,42,44], weights[-,distance] \\
    Tree  & max-depth[5,10,20,50,100], criterion[-,entropy] \\
    SVM   & kernel[linear, poly, rbf, sigmoid], C[0.1,0.5,1,1.5,2.0,2.2,2.4,2.6,2.8,3,4,5], degree[-,2,3], gamma[-,0.005,0.01,0.02,0.05] \\
    Forest & max-depth[10], criterion[-,entropy], n-estimators[5,10,20,50,100] \\
    Logistic & penalty[l1,l2], solver[newton-cg,lbfgs,liblinear,sag,saga], C[0.1,0.2,0.5,1,2,5], tol[0.0001] \\
    Linear & - \\
    Bayes & - \\
    \bottomrule
    \end{tabular}%
  \label{tab:params}%
\end{table*}%


==> data/best_params.tex <==
% Table generated by Excel2LaTeX from sheet 'best_param'
\begin{table}[htbp]
  \centering
	\scriptsize
	\setlength\tabcolsep{2.5pt}
  \caption{The best properties of the machine learning algorithms}
    \begin{tabular}{l|lll}
    \textbf{Alg.} & \textbf{Smpl.} & \textbf{Prec/Rec/F} & \textbf{Best parameters} \\
    \midrule
    \midrule
    DNN$_s$  & $\uparrow$25\% & 0.83/0.62/0.71 & \emph{layers} 5 \emph{neurons} 200 \emph{batch} 100 \emph{epochs} 10 \emph{lr} 0.05 \\
    DNN$_c$  & $\downarrow$25\% & 0.86/0.60/0.71 & \emph{layers} 5 \emph{neurons} 250 \emph{batch} 100 \emph{lr} 0.1 \\
    Forest & $\uparrow$25\% & 0.88/0.63/0.74 & \emph{max-depth} 10 \emph{n-estimators} 100 \\
    KNN   & None  & 0.91/0.66/0.76 & \emph{n\_neighbors} 12 \emph{weights} distance \\
    Lin. reg. & $\uparrow$50\% & 0.57/0.53/0.55 & -- \\
    Log. reg. & $\uparrow$50\% & 0.59/0.55/0.57 & \emph{penalty} l2 \emph{solver} newton-cg \emph{C} 5.0 \emph{tol} 0.0001 \\
    SVM   & $\uparrow$50\% & 0.81/0.65/0.72 & \emph{kernel} rbf C 2.6 \emph{gamma} 0.05 \\
    Tree  & None  & 0.74/0.70/0.72 & \emph{criterion} entropy \emph{max-depth} 100 \\
    Bayes & $\uparrow$75\% & 0.17/0.27/0.21 & -- \\
    \bottomrule
    \end{tabular}%
  \label{tab:best_params}%
\end{table}%


==> js_func_naming.tex <==
In order to determine the functions that were modified by the vulnerability-fixing commits, first we needed a technique to identify the functions in a reliable way to be able to track them across different versions of a project.
It makes it easier to match the vulnerable state of a function with the fixed state, so we can derive valuable information from the changes regarding the fixed vulnerability.
For source code written in JavaScript this task is not so straightforward like, for example, in the case of Java where the fully qualified name of the methods together with the types of its parameters works in almost all cases.
In the large corpus of our JavaScript analysis results, we found that around 50\% of the functions do not have any names assigned to them by the developers, thus they are basically anonymous functions.
%\todoi{ezt a szazalekot pl az elemzett projektekbol lenne erdemes pontositani}
Moreover, functions can be embedded in other functions without any restrictions regarding the depth of the embedding which further complicates this task.
To overcome this obstacle, we applied a heuristic that tries to assign a name to the anonymous functions based on the context of the function declaration.

% title
\emph{Anonymous functions in assignment expressions}.
When an anonymous function is on the right side of an assignment expression, our method tries to produce a name from the left side of the assignment.
We implemented the following naming rules for the assignment expressions.

There is a variable expression on the left side -- in such cases we simply use the name of the referenced variable.
\begin{lstlisting}[language=JavaScript, firstnumber=1, xleftmargin=1cm]
var foo = function(){}; // name: foo
\end{lstlisting}

There is a property accessor on the left side -- in these cases we determine the right-most member of the expression and use its name.
\begin{lstlisting}[language=JavaScript, firstnumber=1, xleftmargin=1cm]
foo.bar.member = function(){}; // name: member
\end{lstlisting}

There is a property accessor with the \textit{this} variable on the left side within an object constructor function.
This is a generic way to add a member function to an object in JavaScript programs.
In these cases we use the name of the referenced member.
\begin{lstlisting}[language=JavaScript, firstnumber=1, xleftmargin=1cm]
function foo() {
  this.bar = function(){}; // name: bar
}
\end{lstlisting}


In JavaScript, the usage of the IIFE design pattern (immediately-invoked function expression) is quite common, where function runs as soon as it is defined.
When such function is on the right side of an assignment expression we apply the same naming rules as in the case of a simple anonymous function declaration.
\begin{lstlisting}[language=JavaScript, firstnumber=1, xleftmargin=1cm]
var foo = (function(){})(); // name: foo
\end{lstlisting}


% title
\emph{Anonymous functions in function call expressions}.
In JavaScript, it is very frequent to pass one or more anonymous functions -- callback functions -- as parameters when calling another function (i.e. higher-order functions).
In such cases we use the name of the invoked function and the sequence number of the parameters (separated by a \$ sign) to name the anonymous functions.
\begin{lstlisting}[language=JavaScript, firstnumber=1, xleftmargin=1cm]
foo(function(){}); // name: foo$0
\end{lstlisting}


% title
\emph{Anonymous functions in Object Literals}.
When an anonymous function is defined inside an object literal as a property (name-value pair) we use the name of the property.
If the object literal is on the right side of an assignment expression, we do not use any assingment related naming rules, but if the object literal is a parameter of a function call, we combine the two naming strategies.
%\todoi{ez utobbi a doksiban nincs jelolve hogy meg lett-e csinalva (object literal parameterkent), Zolitol megkerdezni}
\begin{lstlisting}[language=JavaScript, firstnumber=1, xleftmargin=1cm]
{
  foo: function(){}; // name: foo
}
var foo = {
  bar: function(){} // name: bar
}
foo({
  bar: function(){} // name: foo$0.bar
})
\end{lstlisting}


% title
\emph{Anonymous functions in other cases}.
In all other cases, we apply a general naming rule that simply assigns sequence numbers to the anonymous functions that are local to the parent scope (the containing function if there is one).
\begin{lstlisting}[language=JavaScript, firstnumber=1, xleftmargin=1cm]
function(){
	function(){}; // name: __anonymFunctionExpression0001__
	function(){}; // name: __anonymFunctionExpression0002__
}; // name: __anonymFunctionExpression0001__
\end{lstlisting}


% title
\emph{Avoiding naming conflicts}.
When the same function name is generated by multiple naming rules, name conflict occurs.
The naming strategies previously described do not handle such conflicts.
We implemented a method on top of the naming rules to resolve this problem.
When a name is generated the second time -- local to the scope --, we start indexing them with a counter.
This ensures that no naming conflicts will occur and all the functions will have a unique name.
%\todoi{ezt leellenorizni hogy jol emlekszem-e}
\begin{lstlisting}[language=JavaScript, firstnumber=1, xleftmargin=1cm]
foo(function(){}); // name: foo$0[0]
foo(function(){}); // name: foo$0[1]
\end{lstlisting}


% title
\emph{Assembling a fully qualified name}.
Now that the anonymous functions have a unique name in the local scope, we can use them to assemble a fully qualified name that includes all of the parent functions' names.
We identify each function with its fully qualified name.
\begin{lstlisting}[language=JavaScript, firstnumber=1, xleftmargin=1cm]
function(){
	var foo = function() {
		bar(function(){}); // fully qualified name: __anonymFunctionExpression0001__.foo.bar$0
	};
}; // name: __anonymFunctionExpression0001__
\end{lstlisting}

